Deep Learning for Environmentally Robust Speech Recognition: An Overview of Recent Developments

Eliminating the negative effect of non-stationary environmental noise is a long-standing research topic for automatic speech recognition that stills remains an important challenge. Data-driven supervised approaches, including ones based on deep neural networks, have recently emerged as potential alternatives to traditional unsupervised approaches and with sufficient training, can alleviate the shortcomings of the unsupervised methods in various real-life acoustic environments. In this light, we review recently developed, representative deep learning approaches for tackling non-stationary additive and convolutional degradation of speech with the aim of providing guidelines for those involved in the development of environmentally robust speech recognition systems. We separately discuss single- and multi-channel techniques developed for the front-end and back-end of speech recognition systems, as well as joint front-end and back-end training frameworks.

==> front-end.tex <==
% \documentclass{article}
% 
% \PassOptionsToPackage{dvipsnames}{xcolor}
% \usepackage{tikz}
% \usetikzlibrary{arrows,positioning,fit,petri,backgrounds,decorations.pathmorphing,calc,shapes,shapes.misc, arrows, decorations.markings}
% 
% \usepackage[active,tightpage]{preview}
% \setlength\PreviewBorder{2pt}
% \PreviewEnvironment{tikzpicture}
% 
% \usepackage[latin1]{inputenc}
% 
% \usepackage{amsmath}
% \usepackage{amssymb}
% 
% \begin{document}
% \pagestyle{empty}

\tikzstyle{object} = [rectangle, draw,  text width=1.65cm, minimum height=1.5cm, rounded corners, font=\small, fill=gray!30]
\tikzstyle{action} = [draw, ellipse,  text width=1.5cm,font=\small]
\tikzstyle{symbol} = [text centered, text width=1cm,]

\tikzstyle{arrow0} = [color=gray,->, line width=0.8pt]
\tikzstyle{arrow1} = [color=red,->, line width=0.8pt]
\tikzstyle{arrow2} = [color=blue,->, line width=0.8pt]

\tikzset{every node/.style={inner sep=-3pt,minimum height=0.9cm, text centered}}


\tikzstyle{vecArrow} = [line width=1.4pt,gray, decoration={markings, mark=at position
   1 with {\arrow[line width=1.4pt, gray]{open triangle 60}}},
   double distance=3pt, shorten >= 7pt,
   preaction = {decorate}]


\makebox[\linewidth]{%
\begin{tikzpicture}[>=stealth,node distance = 2.8cm,auto]
    \node[symbol,text width=1.0cm,node distance = 2cm] (signal) {$y(t)$};
    \node[object, right of=signal,node distance = 1.5cm] (prepro) {pre-\\processing};
    \node[object, right of=prepro,node distance = 2cm] (STFT) {Short-Time Fourier Transform}; 
    \node[object, right of=STFT,node distance = 2.5cm] (squared) {square magnitude}; 
    \node[object, right of=squared] (mel) {Mel-\\frequency filterbank};
    \node[object, right of=mel] (logMel) {log Mel-\\frequency filterbank}; 
    \node[object, right of=logMel,node distance = 3.2cm] (DST) {Discrete Cosine Transform}; 
    \node[symbol, right of=DST,node distance = 1.8cm] (MFCC) {$Y^{mfcc}(n)$};
    
    \draw[->] (signal) to (prepro);
    \draw[->] (prepro) -- node[above=-5pt]{}(STFT); 
    \draw[->] (STFT) -- node[above=-5pt]{$Y(n)$}(squared); 
    \draw[->] (squared) -- node[above=-5pt]{$|Y(n)|^2$}(mel);
    \draw[->] (mel) -- node[above=-5pt]{$Y^{mel}(n)$} (logMel); 
    \draw[->] (logMel) -- node[above=-5pt]{$Y^{logMel}(n)$} (DST);
    \draw[->] (DST) to ($(DST.east)+(5mm,0)$);
  
 
\end{tikzpicture}
}

% \end{document}
